SplitOut: Out-of-the-Box Training-Hijacking Detection in Split Learning via Outlier Detection

Split learning enables efficient and privacy-aware training of a deep neural network by splitting a neural network so that the clients (data holders) compute the first layers and only share the intermediate output with the central compute-heavy server. This paradigm introduces a new attack medium in which the server has full control over what the client models learn, which has already been exploited to infer the private data of clients and to implement backdoors in the client models. Although previous work has shown that clients can successfully detect such training-hijacking attacks, the proposed methods rely on heuristics, require tuning of many hyperparameters, and do not fully utilize the clients' capabilities. In this work, we show that given modest assumptions regarding the clients' compute capabilities, an out-of-the-box outlier detection method can be used to detect existing training-hijacking attacks with almost-zero false positive rates. We conclude through experiments on different tasks that the simplicity of our approach we name \textit{SplitOut} makes it a more viable and reliable alternative compared to the earlier detection methods.

==> include/ad_alg.tex <==
\begin{algorithm}[t!]
% \SetAlgoLined
$detected\_attacks$: number of detected attacks for 100 epochs \\ 
$window\_size$: number of gradients in prediction process \\ 
$G$: single gradient list \\ 
$honest\_grads$: honest server gradients\\ 
$no\_of\_neighbors$: one less than the number of length of honest gradients \\ 
\textbf{before} \textit{prediction}, create LOF model with $no\_of\_neighbors$, train LOF with $honest\_grads$  \\

\For{$gradients\_of\_epoch$ from $0$ to $100$}{
        $N \leftarrow random[window\_size: xxx] $ \\ 
        %xxx: 1/3 of length of gradients\_of\_epoch
        
        is\_epoch\_marked = 0 \\
        \For{$G$ from $window\_size$ to $N$}{
            $sub\_gradients \leftarrow gradients\_of\_epoch[G - window\_size: G] $ \\ 

            $ preds \leftarrow \texttt{LOF\_PREDICTION}$(sub\_gradients)$ \\$
            $ no\_of\_inliers \leftarrow \texttt{count\_1}$(sub\_gradients)$ \\$
            $ no\_of\_outliers \leftarrow \texttt{count\_-1}$(sub\_gradients)$ \\$

            \If{$is\_epoch\_marked = 0$}{
                \uIf{$no\_of\_outliers > no\_of\_inliers$}{
                    $is\_epoch\_marked = 1$ \\
                    Increase $detected\_attacks$
                } 
            }
        }
}
\caption{Attack detection with LOF2}
\label{alg:ad}
\end{algorithm}

==> include/ad_results_table.tex <==
\begin{table*}[h!]
    \caption{\textbf{Detecting FSHA Using Anomaly Detection.} True and false positive rates for our AD-based method averaged over 100 runs. AD data rate is the percentage of client data used in simulating the entire model to obtain training data for the LOF algorithm. Window size is the number of most recent single-gradient decisions to perform a majority vote over to reach the final decision. The attack is detected during the first third of the first epoch. Boldface highlights the best combination of shared training data rate for SG-AD and window size in terms of reaching perfect accuracy.}
    \label{tab:ad_full_results}
    \begin{subtable}{0.5\textwidth}
        \caption{True positive rates}
        \label{tab:ad_full_results_tpr}
        \centering
        \begin{tabular}{lcccccccc}
        \toprule
            \textbf{Dataset $\rightarrow$}                & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{F-MNIST} & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100} \\ 
            \textbf{Window Size $\rightarrow$}            & 1    & 10                 & 1      & 10                 & 1      & 10                 & 1      & 10\\ \midrule
            \textbf{AD Data Rate (\%) $\downarrow$}  & \multicolumn{8}{c}{} \\ 
            1                               & 1.0    & \textbf{1.0}                 & 1.0      & \textbf{1.0}                 & 1.0      & \textbf{1.0}                 & 1.0      & \textbf{1.0}\\
            10                              & 1.0    & 1.0                 & 1.0      & 1.0                 & 1.0      & 1.0                 & 1.0      & 1.0\\
            25                              & 1.0    & 1.0                 & 1.0      & 1.0                 & 0.99      & 0.97                 & 1.0      & 1.0\\
            50                              & 1.0    & 1.0                 & 1.0      & 1.0                 & 1.0      & 1.0                 & 1.0      & 0.99\\
            75                             & 1.0    & 1.0                 & 1.0      & 1.0                 & 0.98      & 0.95                 & 0.99      & 1.0\\
            100                             & 1.0    & 1.0                 & 1.0      & 1.0                 & 0.97      & 0.92                 & 1.0      & 1.0\\
        \bottomrule
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.55\textwidth}
        \caption{False positive rates}
        \label{tab:ad_full_results_fpr}
        \centering
        \begin{tabular}{lcccccccc}
        \toprule
            \textbf{Dataset $\rightarrow$}                & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{F-MNIST} & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100} \\ 
            \textbf{Window Size $\rightarrow$}            & 1    & 10                 & 1      & 10                 & 1      & 10                 & 1      & 10\\ \midrule
            \textbf{AD Data Rate (\%) $\downarrow$}  & \multicolumn{8}{c}{} \\ 
            1                               & 0.0    & \textbf{0.0}                 & 0.0      & \textbf{0.0}                 & 0.18      & \textbf{0.0}                 & 0.12      & \textbf{0.0}\\
            10                              & 0.0    & 0.0                 & 0.0      & 0.0                 & 0.01      & 0.0                 & 0.03      & 0.0\\
            25                              & 0.0    & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0\\
            50                              & 0.0    & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0\\
            75                             & 0.0    & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0\\
            100                             & 0.0    & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0                 & 0.0      & 0.0\\
        \bottomrule
        \end{tabular}
    \end{subtable}
\end{table*}

==> include/decision_alg.tex <==
\begin{algorithm}[h!]
\SetKwFunction{func}{MAKE\_DECISION}
\SetKwProg{Fn}{Function}{:}{}

$A$: Model's classification accuracy \\
$A_F$: Expected classification accuracy for a fake batch \\
$B_F$: Share of randomized labels in a fake batch  \\
$N$: Number of initial batches to ignore \\
\Fn{\func{$F, R$}}{
    \uIf{scores are high}{ 
        Keep training.
    } 
    \uElseIf{$A \approx A_F$}{
        \uIf{$B_F = 1$}{
            It is too early to detect. Wait.
        } \Else{
            Increase $B_F$.
        }
        [Optional] Increase $N$.
    }
    \uElse{
        The server is launching an attack. Stop training.
    }
}
\caption{Clients' Decision-Making Process Using SG-LC}
\label{alg:decision}
\end{algorithm}

==> include/main_alg.tex <==
\begin{algorithm}[t!]
% \SetAlgoLined
$f, w$: client model, parameters \\ 
$OPT$: optimizer \\ 
$P_F$: probability of sending fake batches \\ 
$B_F$: number of labels randomized in fake batches \\ 
$N$: number of initial batches to ignore \\
initialize $R_1, R_2, F$ as empty lists \\ 
\texttt{rand}($y$, $B_F$): randomize share $B_F$ of the labels $Y$. \\

\textbf{before} \textit{training}, set parameters $\alpha, \beta, B_F, P_F, T, N$. \\
\While{training}{
    \For{$(x_i,y_i)$ $\leftarrow$ trainset}{
        \uIf{probability $P_{\text{F}}$ occurs \textbf{and} $i \geq N$}{
            // sending fake batches \\
            Send $(f(x_i), \texttt{rand}(y_i, B_F))$ to server \\ 
            Receive gradients $\nabla_F$ from server \\ 
            Append $\nabla_F$ to F \\ 
            \texttt{MAKE\_DECISION}$(F, R_1 \cup R_2)$ \\
            // do not update parameters \\
        }
         \Else {
            // regular training \\
            Send $(f(x_i), y_i)$ to server \\ 
            Receive gradients $\nabla_R$ from server \\ 
            \If{$i \geq N$}{
                \uIf{probability 0.5 occurs}{
                Append $\nabla_R$ to $R_1$
                } \Else {
                    Append $\nabla_R$ to $R_2$
                }
            }
            $w \leftarrow w + OPT(\nabla_R)$ \\
        }
    }
}
\caption{Client training with SG-LC and the label-sharing SplitNN setup}
\label{alg:main}
\end{algorithm}

==> include/od_full_tpr_t_table_FSHA_model2_v2.tex <==
\begin{table*}[ht!]
    % \vspace{-14.00 cm}
    \caption{\textbf{Detecting FSHA using SplitOut \cite{pasquini_unleashing_2021} where different models are used.} True and false positive rates for our method averaged over 100 runs. LOF data rate is the percentage of client data used in simulating the entire model to obtain training data for the LOF algorithm. Window size is the number of most recent single-gradient decisions to perform a majority vote over to reach the final decision. The $t$ field denotes the average point of detection (as the share of total number of batches).}
    \label{tab:ad_full_results}
    \begin{subtable}{1\textwidth}
        \caption{Window size: 1}
        \label{tab:lof_fsha_full_table}
        \centering
        
        \begin{tabular}
        {l|ccc|ccc|ccc|ccc}
        \toprule
        \textbf{Dataset $\rightarrow$} & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{|c|}{\textbf{F-MNIST}} & \multicolumn{3}{c|}{\textbf{CIFAR10}} & \multicolumn{3}{c}{\textbf{CIFAR100}} \\  \textbf{Data Rate $\downarrow$}
                    & TPR & FPR   & $t$    & TPR & FPR & $t$ & TPR & FPR & $t$ & TPR & FPR & $t$  \\ \midrule
        1\%        & 1.0  & 0.0 & 0.0011\pm0.0  & 1.0  & 0.0 & 0.0023\pm0.0002  & 1.0  & 0.98 & 0.0019\pm0.0002  & 1.0  & 0.98 & 0.0014\pm0.0001 \\
        10\%      & 1.0  & 0.0 & 0.0011\pm0.0   & 1.0  & 0.0 & 0.0025\pm0.0002  & 1.0  & 0.96 & 0.0019\pm0.0002 & 1.0  & 0.98 & 0.0014\pm0.0001  \\ 
        25\%      & 1.0  & 0.0 & 0.0011\pm0.0   & 1.0  & 0.0 & 0.0025\pm0.0002  & 1.0  & 0.52 & 0.0044\pm0.0003 & 1.0  & 0.97 & 0.0015\pm0.0001 \\ 
        50\%      & 1.0  & 0.0 & 0.0011\pm0.0   & 1.0  & 0.0 & 0.0025\pm0.0002  & 1.0  & 0.03 & 0.0078\pm0.0002 & 1.0  & 0.43 & 0.0051\pm0.0003  \\
        75\%      & 1.0  & 0.0 & 0.0011\pm0.0   & 1.0  & 0.0 & 0.0025\pm0.0002  & 1.0  & 0.00 & 0.0093\pm0.0003 & 1.0  & 0.04 & 0.0083\pm0.0004 \\
        100\%      & 1.0  & 0.0 & 0.0011\pm0.0   & 1.0  & 0.0 & 0.0025\pm0.0002  & 1.0  & 0.00 & 0.0186\pm0.0011 & 1.0  & 0.00 & 0.0176\pm0.0043 \\
        \bottomrule
        \end{tabular}
    \end{subtable}
    
 
    \vspace*{0.25 cm}
    
    \begin{subtable}{1\textwidth}
        \caption{Window size: 10}

        \centering
        \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \toprule
        \textbf{Dataset $\rightarrow$} & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{|c|}{\textbf{F-MNIST}} & \multicolumn{3}{c|}{\textbf{CIFAR10}} & \multicolumn{3}{c}{\textbf{CIFAR100}} \\  \textbf{Data Rate $\downarrow$}
                    & TPR & FPR   & $t$    & TPR & FPR & $t$ & TPR & FPR & $t$ & TPR & FPR & $t$  \\ \midrule
        1\%        & 1.0  & 0.0 & 0.0107\pm0.0  & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.02 & 0.0128\pm0.0000 & 1.0  & 0.14 & 0.0128\pm0.0000  \\
        10\%      & 1.0  & 0.0 & 0.0107\pm0.0   & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.03 & 0.0128\pm0.0000 & 1.0  & 0.41 & 0.0128\pm0.0000  \\ 
        25\%      & 1.0  & 0.0 & 0.0107\pm0.0   & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.00 & 0.0130\pm0.0001 & 1.0  & 0.14 & 0.0128\pm0.0000 \\ 
        50\%      & 1.0  & 0.0 & 0.0107\pm0.0   & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.00 & 0.0138\pm0.0001 & 1.0  & 0.00 & 0.0134\pm0.0001  \\
        75\%      & 1.0  & 0.0 & 0.0107\pm0.0   & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.00 & 0.0145\pm0.0001 & 1.0  & 0.00 & 0.0173\pm0.0019  \\
        100\%      & 1.0  & 0.0 & 0.0107\pm0.0   & 1.0  & 0.0 & 0.0109\pm0.0001  & 1.0  & 0.00 & 0.0155\pm0.0003 & 1.0  & 0.00 & 0.0308\pm0.0063  \\
      
        \bottomrule
        \end{tabular}
    \end{subtable}
\end{table*}

==> include/policies_alg.tex <==
\begin{algorithm}[t!]
\SetKwFunction{fast}{FAST}
\SetKwFunction{avg}{AVG-K}
\SetKwFunction{voting}{VOTING}
\SetKwProg{Fn}{Function}{:}{}

\Fn{\fast{$S$: scores, $T$: threshold}}{
    \Return $S[-1] < T$
}

\Fn{\avg{$S$: scores,  $k$: number of scores, $T$: threshold}}{
    \Return \texttt{mean}$(S[-k:]) < T$
}

\Fn{\voting{$S$: scores, $n$: group size, $T$: threshold}}{
    votes = 0\\
    c = $\lceil len(scores) / n \rceil $ // group count \\
    // default $c=10$ and $n=5$ \\
    \For{$i$ from $0$ to $c$}{
        group = S[$i \cdot n$ : $(i+1) \cdot n$] \\
        \uIf{\texttt{mean}(group) $< T$}{
            votes += 1 \\
        }
    }
    \Return $votes > c/2$ 
}

\caption{Example Detection Policies for SG-LC}
\label{alg:policies}
\end{algorithm}

==> tables/angles.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/mnist_angles_new.png}
        \caption{MNIST}
        \label{fig:mnist_angle}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/f_mnist_angles_new.png}
        \caption{Fashion-MNIST}
        \label{fig:f_mnist_angle}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar_angles_new.png}
        \caption{CIFAR10}
        \label{fig:cifar_angle}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar100_angles_new.png}
        \caption{CIFAR100}
        \label{fig:cifar100_angle}
    \end{subfigure}
    \caption{\textbf{Comparison of the angle between fake and regular gradients} ($\theta(F,R)$) with the angle between two subsets of regular gradients ($\theta(R_1, R_2)$), averaged over 5 runs during honest training. The x-axis denotes the passage of time during the first training epoch.}
    \label{fig:angles}
\end{figure*}


==> tables/batch_indices.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{lcc}
         \toprule
         \textbf{Dataset} & $\mathbf{N}$ & \textbf{Batch Index} \\ \midrule
         MNIST          & 5  & 14.7 \\ 
         Fashion-MNIST  & 0  & 15.1 \\ 
         CIFAR10        & 50 & 88.6 \\ \bottomrule
    \end{tabular}
    \caption{Average batch indices for which all the subsequent scores are greater than 0.9 with a $B_F$ of 1, averaged over 10 runs. $N$ is the batch index at which the clients start running SplitGuard.}
    \label{tab:batch_indices}
\end{table}

==> tables/detection_results.tex <==
\begin{table*}[h!]
    \centering
     \caption{\textbf{Attack detection statistics using SG-LC and SG-AD}, collected over 100 runs of the first epoch of training with a FSHA attacker and an honest server. The true positive rate (TPR) corresponds to the rate at which SplitGuard succeeds in detecting FSHA. The false positive rate (FPR) corresponds to the share of honest training runs in which SplitGuard mistakenly reports an attack. The $t$ field denotes the average point of detection (as the share of total batches). Boldface highlights the best method for the dataset in terms of reaching perfect (or the highest) accuracy the earliest.}
    \label{tab:detection_results}
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
        \textbf{Method} & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{|c|}{\textbf{F-MNIST}} & \multicolumn{3}{c|}{\textbf{CIFAR10}} & \multicolumn{3}{c}{\textbf{CIFAR100}} \\ \midrule
                    & TPR & FPR   & $t$    & TPR & FPR & $t$ & TPR & FPR & $t$ & TPR & FPR & $t$  \\ \midrule
        LC-Fast        & 1.0   & 0.01  & 0.016  & 1.0  & 0.09 & 0.016  & 1.0  & 0.20 & 0.110  & 1.0  & 0.90 & 0.120  \\
        LC-Avg-10      & 1.0   & 0     & 0.140   & 1.0  & 0.03 & 0.140  & 1.0  & 0.29 & 0.200 & 1.0  & 0.75 & 0.140  \\ 
        LC-Avg-20      & 1.0   & 0     & 0.240   & 1.0  & 0.01 & 0.240  & 1.0  & 0.21 & 0.330 & 1.0  & 0.45 & 0.260  \\ 
        % Avg-50      & 1.0   & 0     & 0.57   & 1.0  & 0    & 0.57  & 1.0  & 0.13 & 0.71 & 1.0  & 0.11 & 0.65  \\
        LC-Voting      & 1.0   & 0     & 0.550   & 1.0  & 0    & 0.550  & 1.0  & 0.02 & 0.700 & 1.0  & 0.11 & 0.650  \\ \midrule
        AD      & \textbf{1.0}   & \textbf{0}     & \textbf{0.011}   & \textbf{1.0}  & \textbf{0}    & \textbf{0.011}  & \textbf{1.0}  & \textbf{0.02} & \textbf{0.013} & \textbf{1.0}  & \textbf{0.02} & \textbf{0.014}  \\        
    \bottomrule
    \end{tabular}
   
\end{table*}

==> tables/emnist-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Detecting FSHA \cite{pasquini_unleashing_2021} using Splitout for EMNIST-digits dataset.} True and false positive rates for our method averaged over 50 runs. LOF data rate is the percentage of client data used in simulating the entire model to obtain training data for the LOF algorithm. Window size is the number of most recent single-gradient decisions to perform a majority vote over to reach the final decision. The $t$ field denotes the average point of detection (as the share of total number of batches). }
\label{tab:emnist-all}
        
\begin{tabular}{@{}c|c|ccc@{}}
\toprule
\textbf{Window Size} & \textbf{Data Rate (\%)} & \textbf{TPR} & \textbf{t}      & \textbf{FPR} \\ \midrule
\multirow{8}{*}{1}   & 0.1                     & 1.0          & 4.1e-06\pm0       & 1.0          \\
                     & 0.29                    & 1.0          & 4.1e-06\pm0       & 0.98         \\
                     & 1                       & 1.0          & 4.1e-06\pm0       & 0.98         \\
                     & 10                      & 1.0          & 4.1e-06\pm0       & 0.94         \\
                     & 25                      & 1.0          & 5.0e-06\pm5.4e-07 & 0.40         \\
                     & 50                      & 1.0          & 9.9e-06\pm1.3e-06 & 0.04         \\
                     & 75                      & 1.0          & 1.4e-05\pm1.6e-06 & 0.00         \\
                     & 100                     & 1.0          & 1.6e-05\pm1.6e-06 & 0.00         \\ \midrule
\multirow{8}{*}{10}  & 0.1                     & 1.0          & 4.1e-06\pm0       & 0.0          \\
                     & 0.29                    & 1.0          & 4.1e-06\pm0       & 0.0          \\
                     & 1                       & 1.0          & 4.1e-06\pm0       & 0.0          \\
                     & 10                      & 1.0          & 4.1e-06\pm0       & 0.0          \\
                     & 25                      & 1.0          & 4.2e-05\pm1.2e-07 & 0.0          \\
                     & 50                      & 1.0          & 4.3e-05\pm4.2e-07 & 0.0          \\
                     & 75                      & 1.0          & 4.3e-05\pm7.4e-07 & 0.0          \\
                     & 100                     & 1.0          & 4.4e-05\pm7.4e-07 & 0.0          \\ \bottomrule
\end{tabular}
\end{table}

==> tables/mags.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/mnist_mag_new.png}
        \caption{MNIST}
        \label{fig:mnist_mag}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/f_mnist_mag_new.png}
        \caption{Fashion-MNIST}
        \label{fig:f_mnist_mag}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar_mag_new.png}
        \caption{CIFAR10}
        \label{fig:cifar_mag}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar100_mag_new.png}
        \caption{CIFAR100}
        \label{fig:cifar100_mag}
    \end{subfigure}
    \caption{\textbf{Comparison of the average magnitude values ($d(F,R)$ and $d(R_1, R_2)$) for fake and regular gradients}, averaged over 5 runs during honest training. The x-axis denotes the passage of time during the first training epoch.}
    \label{fig:mags}
\end{figure*}


==> tables/main_results.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/mnist_main_scores.png}
        \caption{MNIST}
        \label{fig:mnist_results}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/f_mnist_main_scores.png}
        \caption{Fashion-MNIST}
        \label{fig:f_mnist_results}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar10_main_scores.png}
        \caption{CIFAR10}
        \label{fig:cifar_results}
    \end{subfigure}
    \begin{subfigure}{0.25\textwidth}
        \includegraphics[width=\textwidth]{figures/cifar100_main_scores.png}
        \caption{CIFAR100}
        \label{fig:cifar100_results}
    \end{subfigure}
    \caption{\textbf{SG-LC scores obtained} while training with an honest server, and a FSHA attacker until detection during the first epoch, averaged over 5 runs. The x-axis displays the flow of time during the first epoch. The $P_F$ is set to $0.1$, and the $B_F$ values vary when training with an honest server. Lower $B_F$ values are excluded from the CIFAR10/100 results since they do not serve a purpose given the model's classification accuracy. The labels at the end of FSHA lines correspond to the average detection times as the amount of progress within the first epoch, as shown in Table \ref{tab:detection_results} as well.}
    \label{fig:main_results}
\end{figure*}

